Shielding of rotor noise by plates and wings

A method of noise reduction proposed for the next generation of aircraft is to shield noise from the propulsion system, by positioning the noise source over a wing or another surface. In this paper, an approximate analysis is developed for the acoustic field far from a circular source placed near the edge of a semi-infinite plate, a model problem for shielding of noise by a wing and for scattering by a trailing edge. The approximation is developed for a source of small radius and is found to be accurate when compared to full numerical evaluation of the field.

==> Figures/mpxerr.tex <==
\gdef\mpxshipout{\shipout\hbox\bgroup%
  \setbox0=\hbox\bgroup}%
\gdef\stopmpxshipout{\egroup  \dimen0=\ht0 \advance\dimen0\dp0
  \dimen1=\ht0 \dimen2=\dp0
  \setbox0=\hbox\bgroup
    \box0
    \ifnum\dimen0>0 \vrule width1sp height\dimen1 depth\dimen2 
    \else \vrule width1sp height1sp depth0sp\relax
    \fi\egroup
  \ht0=0pt \dp0=0pt \box0 \egroup}
\mpxshipout% line 32 ./jasa2022-figs.mp
$z$%
\stopmpxshipout
\mpxshipout% line 37 ./jasa2022-figs.mp
$y$%
\stopmpxshipout
\mpxshipout% line 38 ./jasa2022-figs.mp
$x$%
\stopmpxshipout
\end{document}

